Kernelization for Treewidth-2 Vertex Deletion

The Treewidth-2 Vertex Deletion problem asks whether a set of at most $t$ vertices can be removed from a graph, such that the resulting graph has treewidth at most two. A graph has treewidth at most two if and only if it does not contain a $K_4$ minor. Hence, this problem corresponds to the NP-hard $\mathcal{F}$-Minor Cover problem with $\mathcal{F} = \{K_4\}$. For any variant of the $\mathcal{F}$-Minor Cover problem where $\mathcal{F}$ contains a planar graph, it is known that a polynomial kernel exists. I.e., a preprocessing routine that in polynomial time outputs an equivalent instance of size $t^{O(1)}$. However, this proof is non-constructive, meaning that this proof does not yield an explicit bound on the kernel size. The $\{K_4\}$-Minor Cover problem is the simplest variant of the $\mathcal{F}$-Minor Cover problem with an unknown kernel size. To develop a constructive kernelization algorithm, we present a new method to decompose graphs into near-protrusions, such that near-protrusions in this new decomposition can be reduced using elementary reduction rules. Our method extends the `approximation and tidying' framework by van Bevern et al. [Algorithmica 2012] to provide guarantees stronger than those provided by both this framework and a regular protrusion decomposition. Furthermore, we provide extensions of the elementary reduction rules used by the $\{K_4, K_{2,3}\}$-Minor Cover kernelization algorithm introduced by Donkers et al. [IPEC 2021]. Using the new decomposition method and reduction rules, we obtain a kernel consisting of $O(t^{41})$ vertices, which is the first constructive kernel. This kernel is a step towards more concrete kernelization bounds for the $\mathcal{F}$-Minor Cover problem where $\mathcal{F}$ contains a planar graph, and our decomposition provides a potential direction to achieve these new bounds.

==> preamble.tex <==
\RequirePackage[ruled]{algorithm2e}
\RequirePackage{amsmath}
\RequirePackage{amssymb}
\RequirePackage{amsthm}
\RequirePackage{subcaption}
\RequirePackage{xurl}
\RequirePackage[numbers]{natbib}
\RequirePackage[margin=1in]{geometry}

\newcommand{\parenthesised}[1]{\left(#1\right)}
\newcommand{\bracketed}[1]{\left[#1\right]}
\newcommand{\braced}[1]{\left\lbrace#1\right\rbrace}
\newcommand{\setdef}[2]{\braced{~#1~\mid~#2~}}
\newcommand{\contract}{/}
\newcommand{\twtwodeletionname}{\textrm{\textsc{TW2D}}}
\newcommand{\twtwodeletionG}[1]{\twtwodeletionname\parenthesised{#1}}
\newcommand{\twtwodeletion}[2]{\twtwodeletionG{#1} \leq #2}
\newcommand{\nottwtwodeletion}[2]{\twtwodeletionG{#1} \not\leq #2}
\newcommand{\treewidth}[1]{\textsc{TW}\parenthesised{#1}}
\newcommand{\treewidthsmallp}[1]{\textsc{TW}(#1)}
\newcommand{\nat}{\mathbb{N}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\bchi}{\chi^{\text{-}1}}
\newcommand{\poly}[1]{\textsc{poly}\parenthesised{#1}}
\newcommand{\polyG}{\poly{|G|}}
\newcommand{\nbound}[1]{\mathcal{#1}\text{-\textsc{bound}}}
\newcommand{\Cbound}[2]{\nbound{C}\parenthesised{#1,#2}}
\newcommand{\Ybound}[2]{\nbound{Y}\parenthesised{#1,#2}}
\newcommand{\Lbound}[3]{\nbound{L}\parenthesised{#1,#2,#3}}
\newcommand{\Pbound}[4]{\nbound{P}\parenthesised{#1,#2,#3,#4}}
\newcommand{\Gbound}[3]{\nbound{G}\parenthesised{#1,#2,#3}}
\newcommand{\bound}[2]{\text{\textsc{bound}}\parenthesised{#1,#2}}

\theoremstyle{definition}
\newtheorem{definition}{Definition}[chapter]
\newtheorem{theorem}{Theorem}[chapter]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{observation}{Observation}[chapter]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{reduction}{Reduction}

% case distinction
\makeatletter
\newcounter{casecounter}
\counterwithin*{casecounter}{corollary}
\newtheoremstyle{casestyle}{5pt}{5pt}{\addtolength{\@totalleftmargin}{15pt}\addtolength{\linewidth}{-15pt}\parshape 1 15pt \linewidth}{}{}{}{ }{\textit{\thmname{#1}}\addtocounter{casecounter}{1}\setcounter{subcasecounter}{0}\setcounter{subsubcasecounter}{0} \thecasecounter\thmnote{~:~#3}.}
\theoremstyle{casestyle}
\newtheorem{case}{Case}

\newcounter{subcasecounter}
\newtheoremstyle{subcasestyle}{5pt}{5pt}{\addtolength{\@totalleftmargin}{30pt}\addtolength{\linewidth}{-15pt}\parshape 1 30pt \linewidth}{}{}{}{ }{\textit{\thmname{#1}}\addtocounter{subcasecounter}{1}\setcounter{subsubcasecounter}{0} \thecasecounter.\thesubcasecounter\thmnote{~:~#3}.}
\theoremstyle{subcasestyle}
\newtheorem{subcase}{Case}

\newcounter{subsubcasecounter}
\newtheoremstyle{subsubcasestyle}{5pt}{5pt}{\addtolength{\@totalleftmargin}{45pt}\addtolength{\linewidth}{-15pt}\parshape 1 45pt \linewidth}{}{}{}{ }{\textit{\thmname{#1}}\addtocounter{subsubcasecounter}{1} \thecasecounter.\thesubcasecounter.\thesubsubcasecounter\thmnote{~:~#3}.}
\theoremstyle{subsubcasestyle}
\newtheorem{subsubcase}{Case}

% inductive cases
\makeatletter
\newtheoremstyle{indcasestyle}{5pt}{5pt}{\addtolength{\@totalleftmargin}{15pt}\addtolength{\linewidth}{-15pt}\parshape 1 15pt \linewidth}{}{}{}{ }{\textit{\thmname{#1}}\addtocounter{casecounter}{1}\setcounter{subcasecounter}{0}\setcounter{subsubcasecounter}{0}\thmnote{~:~#3}.}
\theoremstyle{indcasestyle}
\newtheorem{basecase}{Base case}
\newtheorem{inductivestep}{Inductive step}

\newtheoremstyle{indsubcasestyle}{5pt}{5pt}{\addtolength{\@totalleftmargin}{30pt}\addtolength{\linewidth}{-15pt}\parshape 1 30pt \linewidth}{}{}{}{ }{\textit{\thmname{#1}}\addtocounter{subcasecounter}{1}\setcounter{subsubcasecounter}{0} \thesubcasecounter\thmnote{~:~#3}.}
\theoremstyle{indsubcasestyle}
\newtheorem{indsubcase}{Case}

\newtheoremstyle{indsubsubcasestyle}{5pt}{5pt}{\addtolength{\@totalleftmargin}{45pt}\addtolength{\linewidth}{-15pt}\parshape 1 45pt \linewidth}{}{}{}{ }{\textit{\thmname{#1}}\addtocounter{subsubcasecounter}{1} \thesubcasecounter.\thesubsubcasecounter\thmnote{~:~#3}.}
\theoremstyle{indsubsubcasestyle}
\newtheorem{indsubsubcase}{Case}

